Designing the Game to Play: Optimizing Payoff Structure in Security Games

Effective game-theoretic modeling of defender-attacker behavior is becoming increasingly important. In many domains, the defender functions not only as a player but also the designer of the game's payoff structure. We study Stackelberg Security Games where the defender, in addition to allocating defensive resources to protect targets from the attacker, can strategically manipulate the attacker's payoff under budget constraints in weighted L^p-norm form regarding the amount of change. Focusing on problems with weighted L^1-norm form constraint, we present (i) a mixed integer linear program-based algorithm with approximation guarantee; (ii) a branch-and-bound based algorithm with improved efficiency achieved by effective pruning; (iii) a polynomial time approximation scheme for a special but practical class of problems. In addition, we show that problems under budget constraints in L^0-norm form and weighted L^\infty-norm form can be solved in polynomial time. We provide an extensive experimental evaluation of our proposed algorithms.

==> conclusion.tex <==
\section{Conclusion}
Jointly optimizing payoff structure and resource allocation is common in real-world problems, yet is under-explored in the literature. We provide theoretical and algorithmic results for the joint optimization problem with budget constraint in weighted $L^p$ norm form together with numerical evaluation. 
%In this paper, we provide algorithms with provable approximation guarantee and good practical performance for security games with budget constraint in weighted $L^p$ norm form.
%$L^1$ norm. We also develop $O(n^3)$ and $O(n^2\log n)$ algorithms for budget constraint in $L^0$ and weighted $L^\infty$ norms. We show the superiority of our algorithms against several baselines through extensive numerical evaluation.

==> literature.tex <==
\subsection{Related Work}
Security games have received considerable attention in the literature recently~\cite{Tambe:2011:SGT}, and have seen several successful applications to real-world problems~\cite{Fang:2013:AAMAS:moving,Pita:2008:AAMAS:armor,Fang:2016:AAAI:paws}. Given the game structure, the basic multiple LPs approach to solving for an SSE was developed by~\cite{Conitzer:2006:EC:multipleLP}. \cite{Kiekintveld:2009:AAMAS:origami} propose the efficient ORIGAMI algorithm for games with multiple defender resources. We leverage the insights from both works to devise our algorithms which solves a harder problem. Although many algorithms have been developed to solve security games with various additional properties, in most existing works, the payoff structure is treated as fixed~\cite{Korzhyk:2010:AAAI:multipleresources,Paruchuri:2008:AAMAS:bsg,Laszka:2017:AAAIAICS:alert}, hence neglecting the potential of optimization in this aspect. \cite{Yin:2015:AAAI:dynamicpayoffs} study the security game with dynamic payoffs, yet they do not include the dynamic payoffs into the defender's strategy space. 

Despite its significance, jointly optimizing the payoff structure as well as the resource allocation is under-explored. \cite{Carthy:2016:AAAI:logging} consider the simultaneous optimization of team formation and patrol strategy in network security games. Our work is most directly related to the audit game model~\cite{Blocki:2013:IJCAI:audit1,Blocki:2015:AAAI:audit2}. The idea is that the defender can choose to `audit' a subset of targets, which incurs certain decrease in attacker's penalty for audited targets, quantified as a `punishment rate'. This rate is allowed to be either uniform among targets, or non-uniform. In the end the defender's utility is also decreased because of this punishment rate. A justification they gave is for creating a fearful environment. Compared with their model, ours is more general in the sense that we allow not only manipulation to attacker's penalty, but also attacker's reward. However we assume the manipulation does not affect defender's utility. Moreover, their model allows the addition of complex scheduling constraint, which we do not consider in this paper.

==> literature_audit.tex <==
Blocki et al.~\cite{} also considered a variant of security game called audit games. The idea is that the defender can choose to `audit' a subset of targets, which incurs certain decrease in attacker's penalty for audited targets, quantified as a `punishment rate'. This rate is allowed to be either uniform among targets, or non-uniform. In the end the defender's utility is also decreased because of this punishment rate. A justification they gave is for creating a fearful environment. Compared with their model, ours is more general in the sense that we allow not only manipulation to attacker's penalty, but also attacker's reward. However we assume the manipulation does not affect defender's utility. Moreover, their model allows the addition of complex scheduling constraint, which we do not consider in this paper.
